Fundamental Groups of Genus-$0$ Quadratic Differential Strata via Exchange Graphs

We investigate how exchange-graph techniques can be used to study the topology of strata of meromorphic quadratic differentials. The exchange graph provides natural generators for the fundamental group. By extending the combinatorics of triangulations to weighted mixed-angulations, we generalise the familiar relations arising in the simple-zero case and introduce an additional relation that appears only around higher-order zeroes. In the genus-zero case with four singularities, we show that these relations suffice to give explicit presentations of the fundamental group.

==> 3_Paper_S/Pictures/metric_hexa_1.tex <==
%rays

\foreach \P in {A,B,C,D} {
	\draw[thick] ($(\P -| 0,0) $) -- ($(\P -| 8.5,0) $);
}


%round rays

\draw[thick] (C) arc [start angle=180, end angle=90, x radius=0.5cm, y radius =0.25cm] ;
\coordinate (X) at ( $(C) + (0.5,0.25)$ );
\draw[thick] (X) -- ($(X -| 8.5,0) $) ; 


\draw[thick] (B) arc [start angle=0, end angle=-90, x radius=0.5cm, y radius =0.15cm] ;
\coordinate (X) at ( $(B) + (-0.5,-0.15)$ );
\draw[thick] (X) -- ($(X -| 0,0) $) ; 


\draw[thick] (D) arc [start angle=180, end angle=90, x radius=0.5cm, y radius =0.15cm] ;
\coordinate (X) at ( $(D) + (0.5,0.15)$ );
\draw[thick] (X) -- ($(X -| 8.5,0) $) ; 

\draw[thick] (A) arc [start angle=0, end angle=-90, x radius=0.5cm, y radius =0.25cm] ;
\coordinate (X) at ( $(A) + (-0.5,-0.25)$ );
\draw[thick] (X) -- ($(X -| 0,0) $) ;

%saddles

\draw[red] (B) -- (C);

%\node[left, red, opacity=0.2] at (3.75,5.4) {\small $\hat{\eta}_2$};

\draw[red] (A) --(D);

%\node[left, red] at (2.9,2.75) {\small $\hat{\eta}_{12}$};

\draw[red] (D) -- (B);

%\node[left, red] at (6,4.4) {\small $-\hat{\eta}_2$};

%slits

\path[fill=black,opacity=0.2]
(C) arc [start angle=180, end angle=90, x radius=0.5cm, y radius =0.25cm] -- ( $(C) + (0.5,0)$ );
\coordinate (X) at ( $(C) + (0.5,0.25)$ );
\fill[black,opacity=0.2] ( $(C) + (0.5,0)$ ) rectangle ($(X -| 8.5,0) $);

\path[fill=black,opacity=0.2]
(B) arc [start angle=0, end angle=-90, x radius=0.5cm, y radius =0.15cm] -- ( $(B) + (-0.5,0)$ );
\coordinate (X) at ( $(B) + (-0.5,-0.15)$ );
\fill[black,opacity=0.2] ( $(B) + (-0.5,0)$ ) rectangle ($(X -| 0,0) $);

\path[fill=black,opacity=0.2]
(D) arc [start angle=180, end angle=90, x radius=0.5cm, y radius =0.15cm] -- ( $(D) + (0.5,0)$ );
\coordinate (X) at ( $(D) + (0.5,0.15)$ );
\fill[black,opacity=0.2] ( $(D) + (0.5,0)$ ) rectangle ($(X -| 8.5,0) $);

\path[fill=black,opacity=0.2]
(A) arc [start angle=0, end angle=-90, x radius=0.5cm, y radius =0.25cm] -- ( $(A) + (-0.5,0)$ );
\coordinate (X) at ( $(A) + (-0.5,-0.25)$ );
\fill[black,opacity=0.2] ( $(A) + (-0.5,0)$ ) rectangle ($(X -| 0,0) $);

%zeroes 

\draw[red, thick,fill=white](A)circle(0.22);
\draw[red, thick,fill=white](B)circle(0.22);
\draw[red, thick,fill=white](C)circle(0.22);
\draw[red, thick,fill=white](D)circle(0.22);


==> 3_Paper_S/Pictures/metric_hexa_2.tex <==
%rays

\foreach \P in {A,B,C,D} {
	\draw[thick] ($(\P -| 0,0) $) -- ($(\P -| 8.5,0) $);
}


%round rays

\draw[thick] (C) arc [start angle=0, end angle=90, x radius=0.5cm, y radius =0.25cm] ;
\coordinate (X) at ( $(C) + (-0.5,0.25)$ );
\draw[thick] (X) -- ($(X -| 0,0) $) ; 


\draw[thick] (B) arc [start angle=180, end angle=270, x radius=0.5cm, y radius =0.15cm] ;
\coordinate (X) at ( $(B) + (0.5,-0.15)$ );
\draw[thick] (X) -- ($(X -| 8.5,0) $) ; 


\draw[thick] (D) arc [start angle=0, end angle=90, x radius=0.5cm, y radius =0.15cm] ;
\coordinate (X) at ( $(D) + (-0.5,0.15)$ );
\draw[thick] (X) -- ($(X -| 0,0) $) ; 

\draw[thick] (A) arc [start angle=180, end angle=270, x radius=0.5cm, y radius =0.25cm] ;
\coordinate (X) at ( $(A) + (0.5,-0.25)$ );
\draw[thick] (X) -- ($(X -| 8.5,0) $) ;

%saddles

\draw[red] (B) -- (C);

%\node[left, red, opacity=0.2] at (3.75,5.4) {\small $\hat{\eta}_2$};

\draw[red] (A) -- (D);

%\node[left, red] at (2.9,2.75) {\small $\hat{\eta}_{12}$};

\draw[red] (D) -- (B);

%\node[left, red] at (6,4.4) {\small $-\hat{\eta}_2$};

%slits

\path[fill=black,opacity=0.2]
(C) arc [start angle=0, end angle=90, x radius=0.5cm, y radius =0.25cm] -- ( $(C) + (-0.5,0)$ );
\coordinate (X) at ( $(C) + (-0.5,0.25)$ );
\fill[black,opacity=0.2] ( $(C) + (-0.5,0)$ ) rectangle ($(X -| 0,0) $);

\path[fill=black,opacity=0.2]
(B) arc [start angle=180, end angle=270, x radius=0.5cm, y radius =0.15cm] -- ( $(B) + (0.5,0)$ );
\coordinate (X) at ( $(B) + (0.5,-0.15)$ );
\fill[black,opacity=0.2] ( $(B) + (0.5,0)$ ) rectangle ($(X -| 8.5,0) $);

\path[fill=black,opacity=0.2]
(D) arc [start angle=0, end angle=90, x radius=0.5cm, y radius =0.15cm] -- ( $(D) + (-0.5,0)$ );
\coordinate (X) at ( $(D) + (-0.5,0.15)$ );
\fill[black,opacity=0.2] ( $(D) + (-0.5,0)$ ) rectangle ($(X -| 0,0) $);

\path[fill=black,opacity=0.2]
(A) arc [start angle=180, end angle=270, x radius=0.5cm, y radius =0.25cm] -- ( $(A) + (0.5,0)$ );
\coordinate (X) at ( $(A) + (0.5,-0.25)$ );
\fill[black,opacity=0.2] ( $(A) + (0.5,0)$ ) rectangle ($(X -| 8.5,0) $);

\draw[red, thick,fill=white](A)circle(0.22);
\draw[red, thick,fill=white](B)circle(0.22);
\draw[red, thick,fill=white](C)circle(0.22);
\draw[red, thick,fill=white](D)circle(0.22);

==> packages.tex <==

%languages, pictures
\ProvidesPackage{language}
\usepackage{lmodern}
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\usepackage[english]{babel}
%\usepackage{csquotes}
\usepackage{graphicx,color}
\usepackage[colorlinks, linkcolor=blue!50,anchorcolor=Periwinkle,
citecolor=blue!72,urlcolor=cyan, bookmarksopen,bookmarksdepth=2]{hyperref}
\usepackage[usenames,dvipsnames]{xcolor}
\usepackage{anyfontsize}
\usepackage{comment}
\usepackage{lipsum}

%biblatex
%\usepackage[style=alphabetic,backend=bibtex,maxnames=10]{biblatex}
\usepackage[style=alphabetic,
isbn=false,
doi=false,
url=false,
backend=bibtex,
maxnames=5,
maxalphanames=5,firstinits=true
]{biblatex}
%\usepackage{layout}
\usepackage{enumitem}
\usepackage{afterpage}
%\usepackage{parskip}
\usepackage{aliascnt}
%\usepackage[notref,notcite]{showkeys}
\usepackage{xparse}
\usepackage{caption}
%\usepackage{tabto}
\usepackage{imakeidx}
%\usepackage[normalem]{ulem}
\allowdisplaybreaks


%math
\usepackage{amsmath,amsfonts,amsthm,mathtools,amssymb}
\usepackage{tensor}
\usepackage{amscd,latexsym, mathrsfs, epsfig}
\usepackage{mathdots}
\usepackage{upgreek}
%\usepackage{enumerate}
%\usepackage{undertilde}
\usepackage[all]{xy}
\usepackage{transparent}
%tikz
\usepackage{tikz}
\usepackage{tikz-cd}
\usepackage{float}
\usepackage{circuitikz}
\usetikzlibrary{positioning}
\usetikzlibrary{matrix, calc, arrows, decorations.pathreplacing, decorations.markings, decorations.pathmorphing, backgrounds,fit,positioning,shapes.symbols,chains,shadings,fadings}
\usetikzlibrary{cd}
\usetikzlibrary{intersections}
\tikzset{
	every loop/.style={very thick},
	comp/.style={circle,black,draw,thin,inner sep=0pt,minimum size=5pt,font=\tiny},
	order bottom left/.style={pos=.05,left,font=\tiny},
	order top left/.style={pos=.9,left,font=\tiny},
	order bottom right/.style={pos=.05,right,font=\tiny},
	order top right/.style={pos=.9,right,font=\tiny},
	%
	order middle right/.style={draw,thin,shape=rectangle,inner sep=2pt,outer sep=5pt,pos=.5,right,font=\tiny},
	%
	order middle left/.style={draw,thin,shape=rectangle,inner sep=2pt,outer sep=5pt,pos=.5,left,font=\tiny},
	%	
	order node dis/.style={text width=.75cm},
	circled number/.style={circle, draw, inner sep=0pt, minimum size=12pt},
	below left with distance/.style={below left,text height=10pt},
	below right with distance/.style={below right,text height=10pt}
}

\tikzset{->-/.style={decoration={  markings,  mark=at position #1 with
			{\arrow{>}}},postaction={decorate}}}
\tikzset{-<-/.style={decoration={  markings,  mark=at position #1 with
			{\arrow{<}}},postaction={decorate}}}


\usepackage{array}
\newcolumntype{x}[1]{>{\centering\arraybackslash\hspace{0pt}}p{#1}}
